Rethinking Coherence Modeling: Synthetic vs. Downstream Tasks

Although coherence modeling has come a long way in developing novel models, their evaluation on downstream applications for which they are purportedly developed has largely been neglected. With the advancements made by neural approaches in applications such as machine translation (MT), summarization and dialog systems, the need for coherence evaluation of these tasks is now more crucial than ever. However, coherence models are typically evaluated only on synthetic tasks, which may not be representative of their performance in downstream applications. To investigate how representative the synthetic tasks are of downstream use cases, we conduct experiments on benchmarking well-known traditional and neural coherence models on synthetic sentence ordering tasks, and contrast this with their performance on three downstream applications: coherence evaluation for MT and summarization, and next utterance prediction in retrieval-based dialog. Our results demonstrate a weak correlation between the model performances in the synthetic tasks and the downstream applications, {motivating alternate training and evaluation methods for coherence models.

==> 2.4-LM-task.tex <==
There have been claims that language models (LM) pre-trained on large-scale data produce fluent text that is indistinguishable from those produced by humans \cite{Radford-gpt2}. We propose to evaluate the coherence of such machine-generated texts to assess their readability. We evaluate 100 such machine generated texts from the \red{ two largest LMs}: GPT-2 \cite{radford2019language} and CTRL \cite{keskar2019ctrl}. 


We prompt the LMs with 100 sentences taken from book introductions scraped from the web. However, despite receiving the same prompt, the LMs do not necessarily produce similar content. It would be unfair to compare the coherence evaluations of the texts they produce in such cases. 

To mitigate this problem, we regulate the content produced by the LMs. We do this by interleaving the gold sentences from the book introductions with the LM generated sentences within the prompt. That is, first, the first sentence from the gold data is used to prompt the LMs. The sentence produced by the LM is then extracted. These two sentences are concatenated along with the 3rd sentence from the gold data and used as the next prompt, and so on. This results in a controlled production of text with an equal number of sentences produced by all LMs; every alternate sentence is gold data, and the other half of the text is LM generated. This provides a more robust way to force different LMs to generate similar content, ensuring that the coherence evaluation is more reliable. 


Because of the nature of the texts considered in this task (formal), we use the coherence models that are trained for discriminating WSJ articles. 


==> 4-experiments.tex <==

In this section, we present the performance of the coherence models on standard synthetic tasks (\ie Global/Local Discrimination), followed by the experiments where we apply the coherence models trained on the global discrimination task to three downstream tasks (\ie, abstractive summarization, extractive summarization, and machine translation). We then present the results of the coherence models re-trained on the next utterance ranking task.




For each of the coherence models, we conducted experiments with publicly available codes from the respective authors. The three recent methods use word embeddings: \lexnegrid{}, \transmodel\ and \unimodel\ use Word2vec \cite{Mikolov.Sutskever:13}, average GloVe \cite{pennington2014glove}, and ELMo \cite{PetersELMo:2018} embeddings respectively. We use the default settings and hyperparameters suggested by the authors.



\subsection{Global Discrimination}
\input{4.0-global-dis.tex}

\subsection{Local Discrimination}
\label{res:local-dis}
\input{4.0-local-dis.tex}

\input{4.2-Sum-exp.tex}

\subsection{Machine Translation}
\label{sec:mt-exp}
\input{MT_WSJ}


\subsection{Utterance Ranking}
\input{4.3-Dialog-exp.tex}


















==> 4-experiments_original.tex <==


For each of the coherence models, we conducted experiments with publicly available codes from the respective authors. The three recent methods use word embeddings: \lexnegrid\, \transmodel\ and \unimodel\ use Word2vec \cite{Mikolov.Sutskever:13}, average GloVe \cite{pennington2014glove}, and ELMo \cite{PetersELMo:2018} embeddings respectively. We use the default settings and hyperparameters suggested by the authors.

\subsection{Global Discrimination}
\input{4.0-global-dis.tex}

\subsection{Local Discrimination}
\input{4.0-local-dis.tex}

\subsection{Machine Translation} \label{sec:mt-exp}
\input{4.1-MT-exp.tex}

\input{4.2-Sum-exp.tex}

\subsection{Utterance Ranking}
\input{4.3-Dialog-exp.tex}

\subsection{Evaluation of LM Generated Texts}
\input{4.4-LM-exp.tex}









==> 4.2-Sum-exp_original.tex <==
\subsection{Extractive Summarization}
\label{sub:abs}
\paragraph{Setup.}

We use the test set of CNN/DM for this task. We collected the reference summaries from the CNN/DM test set as well as the summaries generated by the following four state-of-the-art abstractive summarization systems: \Na Pointer-Generator (PG) \citep{See-17}, \Nb {\sc BertSumExtAbs} (BSEA) \citep{Liu2019TextSW}, \Nc UniLM \citep{unilm}, and \Nd SENECA \citep{sharma2019entity}.



{We first conducted a user study to check how often the reference is preferred as a more coherent text over the generated summaries. The agreement between the two annotators was only \textbf{0.54}, showing low preference for the reference summary. Given this, it would not be appropriate to train the models under the assumption that the reference summaries are more coherent. Therefore, we use the coherence models trained on the WSJ dataset for this task as well.}


The coherence models predict the scores for each system-generated summary in the test set. The scores produced by the models are then used to rank the summaries of the same original article. 

We conducted a small-scale human study to validate the effectiveness of the rankings produced by the coherence models. We randomly sampled 10 sets of summaries from the dataset {with each set containing four generated summaries of the same article}, 
thus resulting in $\binom{4}{2} \times 10 = 60$ pairs of {system} summaries. Two annotators were asked to rank each pair of the summaries in terms of coherence; see Appendix for the human study interface.

\paragraph{Results.}


{For the user study, the agreement between the two annotators was \textbf{0.78}, which indicates fairly reliable data.} After we obtain the rankings based on the coherence scores produced by the models, we compute the agreements between the systems and the two annotators, reported in Table \ref{table:sumranking}. \egrid\ and \lexnegrid\ show the highest agreement with human judgements. 

On the right-hand side of Table \ref{table:sumranking}, we present the average ranking of the summaries produced by different summarization models. {This coherence-based evaluation of the summarization systems can be considered a real-world use-case for the coherence models. Each summary is assigned a rank between $1$ and $4$ based on the coherence scores produced by the models.} The average ranking is computed by averaging the rankings over {all the} test samples. It can been seen that the coherence models with higher human agreement, \egrid\ and \lexnegrid\, yield similar rankings; {they rank the summaries produced by UniLM as more coherent than others in general.}





\begin{table}[tb!]
\resizebox{1.01\columnwidth}{!}{%
\begin{tabular}{l|c||cccc}
\toprule 
  & & \multicolumn{4}{c}{\bf{Summarization Systems}} \\ 
 \bf{Models}  & \bf{Agr.} & \bf{BSEA} & \textbf{UniLM} & \textbf{PG} & \bf{SENE} \\

\midrule 
\egrid   & \bf{0.71} & 2.45 & 2.22 & 2.54 & 2.80 \\

\negrid  & 0.68 & 2.13 &  1.89 & 2.84 & 3.13  \\
\lexnegrid   & \bf{0.71}  & 2.52 & 1.97 & 2.88 & 2.62\\
\transmodel & 0.55 & 2.80 & 2.72 & 2.48 & 2.00 \\
\unimodel  & 0.68 & 1.70 & 3.40 & 1.92 & {2.98} \\
\bottomrule 
\end{tabular}
}

\caption{ \textbf{Agr}eement shows the {AC1 agreement for the pairwise ranking of the generated summaries between two annotators and the models. The last four columns show the average rankings ({over the test set}) assigned by the models to the different summarization systems.}}
\label{table:sumranking}
\end{table}


\subsection{Extractive Summarization}

\paragraph{Setup.}

The dataset from \citet{Barzilay:2008} provides 16 sets of summaries where each set corresponds to a multi-document cluster and contains summaries generated by 5 systems and 1 human. The human ratings for these summaries based on coherence  are also available.\footnote{See Appendix for details. Rankings are available in \url{http://homepages.inf.ed.ac.uk/mlap/coherence/}} 



{In this experiment, since there is no agreement between human annotators available, we simply follow the same  experimental setup as in abstractive summarization. We use the coherence models trained on the WSJ dataset to produce scores that can be used to obtain the pairwise ranking of generated summaries.
Based on the ratings provided by \citet{Barzilay:2008}, we can generate the human pairwise rankings.}



\paragraph{Results.}

\begin{table}[t!]
\resizebox{1.01\columnwidth}{!}{%
\begin{tabular}{l|c||ccccc}
\toprule
 & &  \multicolumn{5}{c}{\bf{Summarization Systems}} \\ 
\bf{Models}  & \bf{Agr.} & \bf{S-6} & \textbf{S-13} & \textbf{S-26} & \bf{S-16} & \bf{S-18}\\
\midrule 
\bf{Human Ranking} & -- & 2.31 & 2.44 & 3.88 & 2.75 &  3.63 \\
\midrule 
\egrid  & 0.52 & 2.50 & 3.06 & 3.25 & 3.31 & 2.88 \\

\negrid & \bf{0.70} & 2.31 & 1.75 & 4.13 &  3.31 & 3.50 \\   
\lexnegrid  & 0.57 & 2.63 &  2.63 & 3.31 & 3.31 & 3.13\\
\transmodel & 0.38 & 3.25 & 3.31 & 1.94 & 3.69 & 2.81 \\
\unimodel & 0.35 & 2.94 & 4.38 & 1.63 & 3.31 & 2.75   \\
\bottomrule 
\end{tabular}
}

\caption{{AC1 \textbf{Agr}eement for the pairwise ranking of the generated summaries between human and the models.  The last five columns show the average rankings.}} 
\label{table:exsumranking}
\end{table}



{We present the agreements between the generated human ranking and the systems in Table \ref{table:exsumranking}. We show the average rankings for different extractive systems (\eg \textbf{S-6}, \textbf{S-13}, $\ldots$) in the last five columns. \negrid\ has a higher agreement with human judgement compared to the other models. It also yields an average ranking very similar to the human average ranking. } 



{By showing that models with high human agreements can produce reasonable rankings (see agreements) of summarization systems, we demonstrate that evaluating summarization systems using coherence as a measure is viable as a research objective. We hope that this can serve to motivate summarization evaluation towards the coherence of the summaries rather than purely focusing on the improvements in ROUGE scores.}


